Settling the Horizon-Dependence of Sample Complexity in Reinforcement Learning

Recently there is a surge of interest in understanding the horizon-dependence of the sample complexity in reinforcement learning (RL). Notably, for an RL environment with horizon length $H$, previous work have shown that there is a probably approximately correct (PAC) algorithm that learns an $O(1)$-optimal policy using $\mathrm{polylog}(H)$ episodes of environment interactions when the number of states and actions is fixed. It is yet unknown whether the $\mathrm{polylog}(H)$ dependence is necessary or not. In this work, we resolve this question by developing an algorithm that achieves the same PAC guarantee while using only $O(1)$ episodes of environment interactions, completely settling the horizon-dependence of the sample complexity in RL. We achieve this bound by (i) establishing a connection between value functions in discounted and finite-horizon Markov decision processes (MDPs) and (ii) a novel perturbation analysis in MDPs. We believe our new techniques are of independent interest and could be applied in related questions in RL.

==> martinagle.tex <==
\section{Concentration Inequalities}
In this section we study the concentration inequalities used in previous sections.
\begin{comment}
Before we state our lemma specified to the MDP, we will use the following concentration lemma for martingales, first proved by Feedman \cite{freedman1975tail}.
\begin{theorem}[\cite{tropp2011freedman}, Thm. 1.2]
\label{thm:freedman}
Let $\{X_1, X_2, \ldots, \}$ be a real-valued martingale difference sequence adapted to filtration $\{\cF_0 \subset  \cF_1 \subset   \ldots \}$, i.e.,
$\expect[X_k|\cF_{k-1}]=0$ for $k=1, 2, \ldots $.
%Let $X_k:=Y_k - Y_{k-1}, k=1,2\ldots $ be the difference sequence.
Assume $X_k\le R$ almost surely for all $k\ge 1$ for some $R>0$. 
Define the predictable quadratic variation process of the martingale:
\[
V_k := \sum_{j=1}^k\expect\left[X_j^2\big|\cF_{j-1}\right].
\]
Then for all $t\ge 0$ and $\sigma^2>0$, we have
\[
\Pr\left[\exists k \ge 0: \sum_{j=1}^k X_j\ge t \text{ and } V_k \le \sigma^2\right]
\le\exp\left(-\frac{-t^2/2}{\sigma^2+Rt/3}\right).
\]
\end{theorem}
\end{comment}
\begin{lemma}
\label{lem:upperbound_on_visits}
Suppose a random trajectory 
\[
T=\{(s_0, a_0, r_0), (s_1, a_1, r_1), \ldots, (s_{H-1}, a_{H-1}, r_{H-1}), s_H\}
\]
 is obtained by executing a policy $\pi$.
 For any $(s, a, s') \in \states \times \actions \times \states$,
with probability at least 
$1-\delta$, we have
\[
%\sum_{h=0}^{H-1}X_{s,a, t}
%\le \frac{2\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}X_{s,a, t}\right)+4}{\delta}
%\quad\text{and}\quad
\sum_{h=0}^{H-1}\indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right]
\le \frac{2\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right)+4}{\delta}\cdot P(s'\mid s,a).
\]
\end{lemma}
\begin{proof}
%For a tuple $(s,a, s')\in \states\times \actions\times \states$, let $X_{s,a,s', t}=\indict\left[(s,a, s') = (s_t, a_t, s_{t+1})\right]$ and $X_{s,a,t}=\indict[(s,a) = (s_t, a_t)]$.
%Denote $m:=\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}X_{s,a, t}\right)$ for simplicity.
For each $h \in [H]$, define
\[
I_h = \begin{cases}
1 & h = 0\\
\indict\left[
\sum_{t=0}^{h-1}  \indict\left[(s,a) = (s_t, a_t)\right] \le \qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right)+1\right] & h > 0
\end{cases}.
\]
Let $\mathcal{E}_1$ be the event that for all $h \in [H]$, $I_h =1$.
By definition of $\qtile_{\delta/2}$, 
we have
$
\Pr\left[\mathcal{E}_1\right] \ge 1- \delta/2.
$

For each $h \in [H]$, let $\mathcal{F}_h$ be the filtration induced by $\{(s_0, a_0, r_0), \ldots, (s_{h}, a_{h}, r_{h})\}$.
For each $h \in [H]$, define 
\[X_h = \indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right] \cdot I_h\]
and
\[Y_h = \indict\left[(s,a) = (s_h, a_h)\right] \cdot I_h.\]

When $h = 0$, we have
\[
\expect[X_h] = \expect[\indict\left[(s,a) = (s_0, a_0)\right] \cdot P(s'\mid s,a) = \expect[Y_h] \cdot P(s'\mid s,a) .
\]
When $h \in [H] \setminus \{0\}$, we have
\begin{align*}
\expect[X_h \mid \mathcal{F}_{h - 1}] =& \expect[\indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right] \cdot I_h \mid  \mathcal{F}_{h - 1}] \\
=& \expect[\indict\left[(s,a) = (s_h, a_h)\right] \cdot I_h \mid  \mathcal{F}_{h - 1}]\cdot P(s'\mid s,a),
\end{align*}
which implies 
\[
\expect[X_h] =  \expect[\indict\left[(s,a) = (s_h, a_h)\right] \cdot I_h]\cdot P(s'\mid s,a) =  \expect[Y_h] \cdot P(s'\mid s,a) .
\]
Note that \[\sum_{h = 0}^{H - 1}Y_h \le \qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right) + 2,\] which implies
\[
\expect\left[ \sum_{h =0}^{H - 1} X_h \right] \le \left(  \qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right) + 2 \right) \cdot P(s'\mid s,a) .
\]

By Markov inequality, with probability at least $1-\delta/2$,
\[
 \sum_{h=0}^{H-1}  X_h \le  \frac{2\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right)+4}{\delta}\cdot P(s'\mid s,a).
\]
which we denote as event $\cE_2$.


Conditioned on $\cE_1 \cap \cE_2$ which happens with probability $1-\delta$, we have
\[
\sum_{h=0}^{H-1}\indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right] =\sum_{h=0}^{H-1}  X_h \le  \frac{2\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right)+4}{\delta}\cdot P(s'\mid s,a).
\]
\end{proof}

\begin{lemma}
\label{lemma:martingal_concent}
Suppose a random trajectory 
\[
T=\{(s_0, a_0, r_0), (s_1, a_1, r_1), \ldots, (s_{H-1}, a_{H-1}, r_{H-1}), s_H\}
\]
 is obtained by executing a policy $\pi$.
 For any $(s, a, s') \in \states \times \actions \times \states$,
with probability at least 
$1-\delta$, we have
\begin{align*}
&\left|\sum_{h=0}^{H-1} \indict\left[(s,a, s') = (s_t, a_t, s_{t+1})\right] - P(s'\mid s,a)\cdot \sum_{h=0}^{H-1}\indict\left[(s,a) = (s_t, a_t)\right]\right|\\
\le& \sqrt{\frac{4\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_t, a_t)\right]\right)+8}{\delta}\cdot P(s'\mid s,a)}.
\end{align*}
\end{lemma}
\begin{comment}
\begin{proof}
Denote $m:=\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}X_{s,a, t}\right)$ for simplicity.
We denote $I_0=1$ and for $1\le t\le H$,
$I_h = \mathbb{I}\left(
\sum_{i=0}^{t-1} X_{s,a,t}(T)\le m+1
\right).
$
Let $\mathcal{E}_1$ be the event that there exists $0\le t<H$ with $I_h =0$.
By definition of $\qtile_{\delta}$, 
we have
$
\Pr\left[\mathcal{E}_1\right]
\le \delta.
$

Let $\mathcal{F}_t$ be the filtration induced by the prefix of the trajectory, $\{(s_0, a_0, r_0), \ldots, (s_{t}, a_{t}, r_{t})\}$.
Let $X_t = X_{s,a,s', t}\cdot I_h - P(s'\mid s,a) X_{s,a, t}I_h$.
Obviously, $|X_t|\le 1$.
Notice that 
\begin{align*}
\expect[X_{s,a,s', t}\cdot I_h | \cF_{t-1}] &=
\expect\left\{\expect[X_{s,a,s', t}\cdot I_h|X_{s,a,t}=1,\cF_{t-1}] | \cF_{t-1}\right\}\\
&=
\expect\left\{\expect[X_{s,a, t}\cdot P(s'\mid s,a)\cdot I_h|X_{s,a,t}=1,\cF_{t-1}] | \cF_{t-1}\right\}\\
&=\expect[P(s'\mid s,a)\cdot X_{s,a, t}\cdot I_h | \cF_{t-1}].
\end{align*}
Then we have,
\[
\expect[X_t|\cF_{t-1}]
=\expect[X_{s,a,s', t}\cdot I_h | \cF_{t-1}] - \expect[P(s'\mid s,a)\cdot X_{s,a, t}\cdot I_h | \cF_{t-1}] =0
\]
and
\[
\expect\left[\sum_{h=0}^{H-1}X_t\right] = 0.
\]
Next we bound $\expect[(\sum_{h=0}^{H-1}X_t)^2]$.
Notice that 
\[
\sum_{h=0}^{H-1}X_t
= \sum_{h=0}^{H-1}  X_{s,a,s', t}\cdot I_h - P(s'\mid s,a)\sum_{h=0}^{H-1}  X_{s,a, t}\cdot I_h.
\]

Next, we bound the conditional variance: $V_t := \sum_{k=1}^t\expect[X_k^2|\cF_{k-1}]$.
Note that
\begin{align*}
X_t^2 &= (X_{s,a,s', t}\cdot I_h - P(s'\mid s,a)\cdot X_{s,a, t}\cdot I_h)^2 \\
&=
I_h \cdot (X_{s,a,s', t} - P(s'\mid s,a)\cdot X_{s,a, t})^2\\
&\le 
I_h\cdot (X_{s,a,s', t}^2 + 
P(s'\mid s,a)^2\cdot X_{s,a, t}^2)\\
&\le 
I_h\cdot (X_{s,a,s', t} + 
P(s'\mid s,a)^2\cdot X_{s,a, t}).
\end{align*}
Hence we have
\begin{align*}
V_t
&\le \sum_{k=1}^t\expect[I_k\cdot X_{s,a,s', k} 
+ I_k\cdot P(s'\mid s,a)^2\cdot X_{s,a, k}
|\cF_{k-1}]\\
&=\sum_{k=1}^t\expect[I_k\cdot X_{s,a, k}\cdot P(s'\mid s,a) 
+ I_k\cdot X_{s,a, k}\cdot P(s'\mid s,a)^2
|\cF_{k-1}].
\end{align*}
Note that
\begin{align*}
\expect[V_t]
 &= 
 \expect\left(\sum_{k=1}^t\expect[I_k\cdot X_{s,a, k}\cdot P(s'\mid s,a) 
+ I_k\cdot X_{s,a, k}\cdot P(s'\mid s,a)^2
|\cF_{k-1}]\right)\\
&=
 \expect\left(\sum_{k=1}^tI_k\cdot X_{s,a, k}\cdot P(s'\mid s,a) 
+ I_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a)^2\right)\\
&\le 
 \expect\left(\sum_{k=1}^tI_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a) 
+ I_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a)^2\right)\\
&\le 
2(m+1)\cdot P(s'\mid s,a).
\end{align*}
Let the $\cE_2$ be the event that 

\end{proof}
\end{comment}



\begin{proof}
For each $h \in [H]$, define
\[
I_h = \begin{cases}
1 & h = 0\\
\indict\left[
\sum_{t=0}^{h-1}  \indict\left[(s,a) = (s_t, a_t)\right] \le \qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right)+1\right] & h > 0
\end{cases}.
\]
Let $\mathcal{E}_1$ be the event that for all $h \in [H]$, $I_h =1$.
By definition of $\qtile_{\delta/2}$, 
we have
$
\Pr\left[\mathcal{E}_1\right] \ge 1- \delta/2.
$

For each $h \in [H]$, let $\mathcal{F}_h$ be the filtration induced by $\{(s_0, a_0, r_0), \ldots, (s_{h}, a_{h}, r_{h})\}$.
For each $h \in [H]$, define
\[
X_h =  \indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right]  \cdot I_h - P(s'\mid s,a)  \indict\left[(s,a) = (s_h, a_h)\right]  \cdot I_h.
\]
As we have shown in the proof of Lemma~\ref{lem:upperbound_on_visits}, for each $h \in [H]$, $\expect[X_h] = 0$.
Moreover, for any $0\le h'< h\le H-1$, we have
\[
\expect[X_h X_{h'}]
= 
\expect[\expect[X_hX_{h'}|\cF_{h-1}]]
=\expect[X_{h'}\expect[X_h|\cF_{h-1}]] = 0.
\]
Therefore,
\[
\expect\left[\left(\sum_{h=0}^{H-1}X_h\right)^2\right]
= \expect\left[\sum_{h=0}^{H-1}X_h^2\right].
\]
Note that for each $h \in [H]$.
\begin{align*}
X_h^2 &= (\indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right]  \cdot I_h - P(s'\mid s,a)  \indict\left[(s,a) = (s_h, a_h)\right]  \cdot I_h)^2 \\
& \le
I_h\cdot \left(\indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right] + 
\left(P(s'\mid s,a)\right)^2\cdot  \indict\left[(s,a) = (s_h, a_h)\right]  \right).
\end{align*}
As we have shown in the proof of Lemma~\ref{lem:upperbound_on_visits}, for each $h \in [H]$, 
\[
\expect[I_h\cdot \indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right]]  = \expect[I_h\cdot \indict\left[(s,a) = (s_h, a_h)\right]] \cdot P(s'\mid s,a),
\]
which implies
\begin{align*}
\expect\left[\left(\sum_{h=0}^{H-1}X_h\right)^2\right] &= \expect\left[\sum_{h=0}^{H-1}X_h^2\right]\\
&\le \sum_{h=0}^{H-1} \expect\left[I_h\cdot \left(\indict\left[(s,a, s') = (s_h, a_h, s_{h+1})\right] + 
\left(P(s'\mid s,a)\right)^2\cdot  \indict\left[(s,a) = (s_h, a_h)\right]  \right)\right]\\
&\le 2   P(s'\mid s,a) \cdot \sum_{h=0}^{H-1} \expect\left[ I_k\cdot  \indict\left[(s,a) = (s_h, a_h) \right]\right]\\
&\le 
2  P(s'\mid s,a) \cdot \left(\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_h, a_h)\right]\right) +2\right).
\end{align*}
By Chebyshev's inequality, we have with probability at least $1-\delta/2$,
\[
\left|\sum_{h = 0}^{H - 1}X_h\right| \le 
 \sqrt{\frac{4\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_t, a_t)\right]\right)+8}{\delta}\cdot P(s'\mid s,a)}.
\]
which we denote as event $\cE_2$.

Conditioned on $\cE_1\cap \cE_2$ which happens with probability $1-\delta$, we have
\begin{align*}
&\left|\sum_{h=0}^{H-1} \indict\left[(s,a, s') = (s_t, a_t, s_{t+1})\right] - P(s'\mid s,a)\cdot \sum_{h=0}^{H-1}\indict\left[(s,a) = (s_t, a_t)\right]\right|\\
\le& \sqrt{\frac{4\qtile_{\delta/2}\left(\sum_{h=0}^{H-1}\indict\left[(s,a) = (s_t, a_t)\right]\right)+8}{\delta}\cdot P(s'\mid s,a)}.
\end{align*}
\begin{comment}
Note that
\begin{align*}
\expect[V_t]
 &= 
 \expect\left(\sum_{k=1}^t\expect[I_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a) 
+ I_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a)^2
|\cF_{k-1}]\right)\\
&=
 \expect\left(\sum_{k=1}^tI_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a) 
+ I_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a)^2\right)\\
&\le 
 \expect\left(\sum_{k=1}^tI_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a) 
+ I_k\cdot X_{s,a, k}\cdot P(s'\mid  s,a)^2\right)\\
&\le 
2(m+1)\cdot P(s'\mid  s,a).
\end{align*}
Let the $\cE_2$ be the event that 
\end{comment}
\end{proof}
%
\begin{lemma}[Probability Approximation Error]
Suppose a $D=\{(s_t^{(k)}, a_t^{(k)})_{h=0}^{H-1}\}_{k=1}^{K}$ is a set of state-action tuples collected by rolling out a policy $\pi$ for some $K>0$ episodes, with initial distribution $\mu$.
For a $(s,a, s')\in \states\times\actions\times\states$,
let \[
\widehat{P}(s'\mid s,a) = \frac{\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}, s_{t+1}^{(k)}) = (s,a,s')\right)}{\max\left[\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)})= (s,a)\right), 1\right]}
\]
be the empirical estimator for $P(s'|s,a)$.
Suppose $K\delta\ge 64\log(4/\delta)$, 
$\qtile^{\pi}_{\mu,\delta/4}(s,a)\ge 1$.
Then with probability at least $1-\delta$,
\[
\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)\ge \frac{K\delta\cdot \qtile^{\pi}_{\mu,\delta/4}(s,a)}{8},
\]
\[
|\widehat{P}(s'\mid s,a) - P(s'\mid s,a)| 
\le   \sqrt{\frac{32\cdot P(s'\mid  s,a)}{\delta\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}}
\le 
\sqrt{\frac{256\cdot P(s'\mid  s,a)}{ K\cdot  \qtile^{\pi}_{\mu,\delta/4}(s,a)\cdot\delta^2}},
\]
and
%, if $P(s'\mid s,a)\ge \frac{1920}{\delta^2\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}$,
%then, 
%with probability at least $1-\delta$,
\[
|\widehat{P}(s'\mid s,a) - P(s'\mid s,a)| 
\le   \min\left(\sqrt{\frac{64\cdot \widehat{P}(s'\mid  s,a)}{\delta^2\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}}
,
\frac{64}{\delta\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}
\right).
 \]
\end{lemma}
\begin{proof}
Using the same proof in Lemma~\ref{lemma:martingal_concent}, we have,
with probability at least $1-\delta/4$,
\begin{align*}
&\left|\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}, s_{t+1}^{(k)})  = (s,a,s')\right) - P(s'\mid s,a )\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)\right| \\
&\le 
\sqrt{\frac{16(m_K+2)\cdot P(s'\mid  s,a)}{\delta}},
\end{align*}
which we denote as event $\cE_1$, where $m_K = \qtile_{\delta/8}\left(\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)\right)$.
Hence we have, with probability at least $\delta/8$,
\[
\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right) \ge  m_K,
\]
which we denote as event $\cE_2$.
Next, we show that $\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)$ is not too small.
Let $m=\qtile^{\pi}_{\mu, \delta/4}(s,a)$.
Let $Y_k$ be the indicator that 
$\sum_{t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)\ge m$.
 by definition of $m$, we have $\Pr[Y_k=1]\ge \delta/4$.
By Chernoff bound, we have
\[
\Pr\left[\sum_k Y_k \le \frac{K\delta}{8}\right]
\le \exp\left(-\frac{(K\delta/8)^2}{K\delta}\right)
= \exp\left(-\frac{K\delta}{64}\right)
\le \frac{\delta}{4}.
\]
Thus with probability at least $1-\delta/4$,
\[
\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)
\ge \frac{Km\delta}{8}\ge 1
\]
which we denote as $\cE_3$,
Hence,  on $\cE_1\cap \cE_2\cap \cE_3$, which happens with probability at least $1-\delta$,
\begin{align*}
\left|\widehat{P}(s'\mid s,a) - {P}(s'\mid s,a)\right|
 &= 
 \frac{\left|\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}, s_{t+1}^{(k)})  = (s,a,s')\right) - P(s'\mid s,a )\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)\right|}{\sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}
 \\
 &\le 
  \sqrt{\frac{16(m_K+2)\cdot P(s'\mid  s,a)}{\left( \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)\right)^2}}\\
  &\le 
  \sqrt{\frac{32\cdot P(s'\mid  s,a)}{\delta\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}}
 \\
 &\le \sqrt{\frac{256\cdot P(s'\mid  s,a)}{ K m\delta^2}}.
\end{align*}
Lastly,  if $P(s'\mid s,a)\ge \frac{128}{\delta\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}$,
then, 
with probability at least $1-\delta$,
\[
|\widehat{P}(s'\mid s,a) - P(s'\mid s,a)| 
\le  P(s'\mid s,a) /2.
\]
Hence,
\[
|\widehat{P}(s'\mid s,a) - P(s'\mid s,a)| 
\le  \sqrt{\frac{64\cdot \widehat{P}(s'\mid  s,a)}{\delta\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)}}.
\]
Otherwise,
\[
|\widehat{P}(s'\mid s,a) - P(s'\mid s,a)| 
\le  
\frac{64}{\delta\cdot \sum_{k,t}\indict\left((s_t^{(k)}, a_t^{(k)}) = (s,a)\right)},
\]
with probability $1-\delta$.
\end{proof}
